Locally Orderless Images for Optimization in Differentiable Rendering

Problems in differentiable rendering often involve optimizing scene parameters that cause motion in image space. The gradients for such parameters tend to be sparse, leading to poor convergence. While existing methods address this sparsity through proxy gradients such as topological derivatives or lagrangian derivatives, they make simplifying assumptions about rendering. Multi-resolution image pyramids offer an alternative approach but prove unreliable in practice. We introduce a method that uses locally orderless images, where each pixel maps to a histogram of intensities that preserves local variations in appearance. Using an inverse rendering objective that minimizes histogram distance, our method extends support for sparsely defined image gradients and recovers optimal parameters. We validate our method on various inverse problems using both synthetic and real data.

==> figures/fig10.tex <==
\begin{figure}
    \def\svgwidth{\columnwidth}
    \small
\input{assets/fig10.pdf_tex}
\caption{
\label{fig:texture} \textbf{Texture Recovery.} Starting from a random
initialization, we recover a reference texture using $\beta=1/8$. We compare our
histogram-space blurring approach ($\alpha=5,\sigma=0$) with standard
$\sigma$-space blurring ($\alpha=0, \sigma=5$). The $\sigma$-space matching
yields suboptimal results since it only measures errors in the means of the
distributions.}
\end{figure}


==> figures/fig11.tex <==
\begin{figure}[h!]
    \def\svgwidth{\columnwidth}
    \small
\input{assets/fig11.pdf_tex}
\caption{
\label{fig:beta} Our method remains robust to different choices of the
$\beta$-kernel width when recovering a textured plane. We demonstrate this by
comparing image error plots across two different kernel widths, both of which
converge to good local minima.}
\end{figure}


==> figures/fig12.tex <==
\begin{figure*}
    \def\svgwidth{0.95\textwidth}
    \small
    \input{assets/fig12.pdf_tex}
    \caption{ \label{fig:timing} \textbf{Runtime Analysis.} We measure the
    effects of kernel-width parameters ($\alpha$, $\beta$, and $\sigma$) on the
    total runtime of computing LOIs. The runtime increases linearly with kernel
    width, with histogram-space blurring ($\alpha$ kernels) being the slowest
    operation. }
\end{figure*}


==> figures/fig13.tex <==
\begin{figure*}
    \def\svgwidth{0.95\textwidth}
    \small
    \input{assets/fig13.pdf_tex}
    \caption{ 
    \label{fig:histogram} \textbf{Histogram visualization.} We visualize the
    histogram contributions across the three color channels at different $\alpha$
    kernel widths. While standard Gaussian Pyramids only preserve the mean of
    each distribution, our method preserves their modes.
    }
\end{figure*}


==> figures/fig14.tex <==
\begin{figure}
    \def\svgwidth{\columnwidth}
    \small
\input{assets/fig14.pdf_tex}
\caption{
\label{fig:beta_only} \textbf{Ablation on $\alpha, \sigma$.} The parameter
$\beta$ alone does not influence the support of RGB gradients. When used in
isolation without the $\alpha$ and $\sigma$ spaces, the optimization converges
to poor local minima. We demonstrate this by attempting to recover disk
positions from random initializations using only $\beta$ scale space.}
\end{figure}


==> figures/fig15.tex <==
\begin{figure}
    \def\svgwidth{\columnwidth}
    \small
\input{assets/fig15.pdf_tex}
\caption{
\label{fig:rasterization} \textbf{Visual comparisons on rasterization
benchmark.} We show visual comparisons on three tasks from the rasterization
benchmark in~\cite{xingDifferentiableRenderingUsing2022}.}
\end{figure}


==> figures/fig8.tex <==
\begin{figure*}
    \def\svgwidth{0.95\textwidth}
    \small
    \input{assets/fig8.pdf_tex}
    \caption{ 
    \label{fig:path2} \textbf{More comparisons on Differentiable Path Tracing.}
    We show additional comparisons with GP~\cite{adelson1984pyramid} and
    MS-SSIM~\cite{wang2003multiscale} along with Error plots (Image MSE \vs Iterations) for each scene in Figure 7 in the main manuscript.
    }
\end{figure*}


==> figures/fig9.tex <==
\begin{figure*}
    \def\svgwidth{0.95\textwidth}
    \small
    \input{assets/fig9.pdf_tex}
    \caption{ 
    \label{fig:disks2} \textbf{2D Comparisons.} We show convergence plots (Image MSE \vs Iterations) and
    optimized results for the 2D benchmark task of optimizing disk positions 
    (Table 1 and Figure 6 in the main manuscript).
    }
\end{figure*}

